Web APIs in Android through the Lens of Security

Web communication has become an indispensable characteristic of mobile apps. However, it is not clear what data the apps transmit, to whom, and what consequences such transmissions have. We analyzed the web communications found in mobile apps from the perspective of security. We first manually studied 160 Android apps to identify the commonly-used communication libraries, and to understand how they are used in these apps. We then developed a tool to statically identify web API URLs used in the apps, and restore the JSON data schemas including the type and value of each parameter. We extracted 9,714 distinct web API URLs that were used in 3,376 apps. We found that developers often use the java.net package for network communication, however, third-party libraries like OkHttp are also used in many apps. We discovered that insecure HTTP connections are seven times more prevalent in closed-source than in open-source apps, and that embedded SQL and JavaScript code is used in web communication in more than 500 different apps. This finding is devastating; it leaves billions of users and API service providers vulnerable to attack.

==> preamble.tex <==
% !TEX root = web-api.tex

%\IEEEoverridecommandlockouts
% The preceding line is only needed to identify funding in the first footnote. If that is unneeded, please comment it out.
% \usepackage{cite}
% \usepackage{amsmath,amssymb,amsfonts}
% \usepackage{algorithmic}
% \usepackage{graphicx}
% \usepackage{textcomp}
% \usepackage{xcolor}

\usepackage{amsthm}
\usepackage{xspace}
%\usepackage{float}
\usepackage{ifthen}
%\usepackage{amsbsy}
\usepackage{amssymb}
\usepackage{balance} % for balancing last page reference column
%\usepackage{booktabs}
%\usepackage{graphicx}
%\usepackage{rotating}
%\usepackage{multirow}
%\usepackage{needspace}
%\usepackage{microtype}
%\usepackage{bold-extra}
%\usepackage{geometry}
%\usepackage{varioref}
%\usepackage{xcolor}
%\usepackage{textcomp}
\usepackage{listings}
\usepackage[normalem]{ulem} %emphasize still italic
%\usepackage{ucs}
%\usepackage{times}
%\usepackage{url}
%\usepackage{alltt}
\usepackage{amsmath}
%\usepackage{xfrac}
%\usepackage{subfigure}
%\usepackage{stmaryrd}   % for the \shortuparrow
%\usepackage{setspace}
%\usepackage[numbers, sort&compress]{natbib}
%\usepackage{mdwlist}        % support for better spaced lists
%\usepackage{chngpage} % allows for temporary adjustment of side margins
%\usepackage[normalem]{ulem} 
\usepackage{array, booktabs}
%\usepackage{balance}
%\usepackage{xspace}
%\PassOptionsToPackage{hyphens}{url}
\usepackage[pdftex,colorlinks=true,pdfstartview=FitV,linkcolor=black,citecolor=black,urlcolor=black]{hyperref}
%\usepackage{needspace}
\usepackage{ifthen}
%\usepackage[normalem]{ulem} % for \sout
%\usepackage{xcolor}
\usepackage[most]{tcolorbox}
%\usepackage{textcomp}
\usepackage{listings}
%\usepackage[multiple]{footmisc}
\usepackage[caption=false]{subfig}
%\usepackage{subfloat}
%\usepackage{arydshln} % for cdashline
\usepackage{paralist} %to list extends of previous work
%deactivate indentation on new paragraphs
%\usepackage{parskip}
% for wrapping text in table cells
%\usepackage{tabularx}
\usepackage{fontawesome}      % for icon next to scg URL next to author list on title page
\usepackage{adjustbox} 		% for vertical text in tables
\usepackage{pifont} 		% for crosses and ticks in tables
\usepackage{algorithm}
\usepackage{algpseudocode}
\algtext*{EndIf}
\algtext*{EndFor}

\newcolumntype{R}[2]{
    >{\adjustbox{angle=#1,lap=\width-(#2),margin*=0.4em 0em 0em 0em}\bgroup}
    l
    <{\egroup}
}
\newcommand*\rot{\multicolumn{1}{R{90}{1em}}} % no optional argument here, please!

% for footnotes 1,2,3..... style
% (traditional approach with \usepackage[multiple]{footmisc} breaks clickable links, overrides behavior)
\let\oldFootnote\footnote
\newcommand\nextToken\relax
\renewcommand\footnote[1]{%
    \oldFootnote{#1}\futurelet\nextToken\isFootnote}
\newcommand\isFootnote{%
    \ifx\footnote\nextToken\textsuperscript{,}\fi}

% only used for theses
%\usepackage{appendix}
%\usepackage[utopia]{quotchap}


%\subfiglabelskip=0pt

\renewcommand{\arraystretch}{1.2}

\newcommand{\needlines}[1]{\Needspace{#1\baselineskip}}
\newcommand{\ra}{$\rightarrow$}
\newcommand{\id}[1]{$-$Id: scgPaper.tex 32478 2010-04-29 09:11:32Z oscar $-$}
\newcommand{\yellowbox}[1]{\fcolorbox{gray}{yellow}{\bfseries\sffamily\scriptsize#1}}
\newcommand{\triangles}[1]{{\sf\small$\blacktriangleright$\textit{#1}$\blacktriangleleft$}}
\newcommand{\nb}[2]{\nbc{#1}{#2}{orange}}
\newcommand{\here}{\yellowbox{$\Rightarrow$ CONTINUE HERE $\Leftarrow$}}
\newcommand\rev[2]{\nb{TODO (rev #1)}{#2}} % reviewer comments
\newcommand\fix[1]{\nb{FIX}{#1}}
\newcommand\todo[1]{\nb{TO DO}{#1}}
\newcommand\on[1]{\nbc{ON}{#1}{olive}} % add more author macros here
\newcommand\nm[1]{\nbc{NM}{#1}{red}}
\newcommand\mg[1]{\nbc{MG}{#1}{purple}}
\newcommand\pg[1]{\nbc{PG}{#1}{violet}}
\newcommand\np[1]{\nbc{NP}{#1}{green}}
\newcommand\pr[1]{\nbc{PR}{#1}{blue}}
\newcommand\ml[1]{\nbc{ML}{#1}{brown}}
\newcommand\cc[1]{\nbc{CC}{#1}{orange}}
\newcommand\pf[1]{\nbc{PF}{#1}{magenta}}
\newcommand\msg[1]{\nbc{MESSAGE}{#1}{brown}}
\newcommand\fw[1]{\nbc{FUTUREWORK}{#1}{black}}
\newcommand\remind[1]{\nbc{REMINDER}{#1}{gray}}
\newcommand\review[1]{\nbc{TO REVIEW}{#1}{orange}}
\newcommand\rA[1]{\nbe{Reviewer 1}{#1}{cyan}}
\newcommand\rB[1]{\nbe{Reviewer 2}{#1}{olive}}
\newcommand\rC[1]{\nbe{Reviewer 3}{#1}{magenta}}
\newcommand\rD[1]{\nbe{Reviewer 4}{#1}{orange}}
\newcommand\ANS[1]{\nbe{Response}{#1}{teal}}
\newcommand\meta[1]{\nbe{Metareview}{#1}{red}}
\newcommand{\ie}{\emph{i.e.},\xspace}
\newcommand{\eg}{\emph{e.g.},\xspace}
\newcommand{\etal}{\emph{et al.}\xspace}
\newcommand{\etc}{\emph{etc.}\xspace}
\newcommand{\smell}[1]{\textbf{#1}.}
\newcommand{\Issue}{\emph{Issue:}\xspace}
\newcommand{\Consequences}{\emph{Consequently},\xspace}
\newcommand{\consequences}{\emph{consequently},\xspace}
\newcommand{\Symptoms}{\emph{Symptom:}\xspace}
\newcommand{\Mitigation}{\emph{Mitigation:}\xspace}
\newcommand{\Detection}{\emph{Detection:}\xspace}
\newcommand{\Limitations}{\emph{Limitation:}\xspace}

\newcommand{\secheaderfield}[1]{\textbf{\code{#1}}}
\newcommand{\Use}{\emph{Use:}\xspace}
\newcommand{\Default}{\emph{If not used},\xspace}
\newcommand{\Risk}{\emph{Risk:}\xspace}
\newcommand{\Adaptation}{\emph{Adaptation:}\xspace}
\newcommand{\SecGain}{\emph{Security Gain:}\xspace}

\newcommand{\yes}{\ding{52}}
\newcommand{\no}{\ding{54}}

\newcommand{\n}{$\cdot$}
\newcommand{\y}{\checkmark}
\newcommand{\subscript}[1]{$_{\textrm{\footnotesize{#1}}}$}
\newcommand{\superscript}[1]{$^{\textrm{\footnotesize{#1}}}$}
\newcommand{\vertical}[1]{\raisebox{-4em}{\begin{sideways}{#1}\end{sideways}}}
\newcommand{\code}[1]{\texttt{#1}}
\newcommand{\paratitle}[1]{\emph{#1. }}

\newcolumntype{L}[1]{>{\raggedright\arraybackslash}m{#1}} % left aligned column

% given by IEEE template
\def\BibTeX{{\rm B\kern-.05em{\sc i\kern-.025em b}\kern-.08em
	T\kern-.1667em\lower.7ex\hbox{E}\kern-.125emX}}
	
% ============================================================
% Markup macros for proof-reading
\newboolean{showedits}
\setboolean{showedits}{true} % toggle to show or hide edits
\ifthenelse{\boolean{showedits}}
{
	\newcommand{\meh}[1]{\textcolor{red}{\uwave{#1}}} % please rephrase
	\newcommand{\ins}[1]{\textcolor{blue}{\uline{#1}}} % please insert
	\newcommand{\del}[1]{\textcolor{red}{\sout{#1}}} % please delete
	\newcommand{\chg}[2]{\textcolor{red}{\sout{#1}}{\ra}\textcolor{blue}{\uline{#2}}} % please change
	\newcommand{\nbe}[3]{
		{\colorbox{#3}{\bfseries\sffamily\scriptsize\textcolor{white}{#1}}}
		{\textcolor{#3}{\sf\small$\blacktriangleright$\textit{#2}$\blacktriangleleft$}}}
}{
	\newcommand{\meh}[1]{#1} % please rephrase
	\newcommand{\ins}[1]{#1} % please insert
	\newcommand{\del}[1]{} % please delete
	\newcommand{\chg}[2]{#2}
	\newcommand{\nbe}[3]{}
}


% ============================================================
% Box comments/edits
\ifthenelse{\boolean{showedits}}
{
	\newtcolorbox{inserted}{
		title=Inserted text:,
		colframe=blue,colback=blue!5!white,
		breakable,
		leftrule=0mm, 
		bottomrule=0mm,
		rightrule=0mm,
		toprule=0mm,
		arc=0mm, outer arc=0mm,
		oversize
	}
	\newtcolorbox{deleted}{
		title=Deleted text:,
		colframe=red,colback=red!5!white,
		breakable,
		leftrule=0mm, 
		bottomrule=0mm,
		rightrule=0mm,
		toprule=0mm,
		arc=0mm, outer arc=0mm,
		oversize
	}
	\newtcolorbox{refactored}{
		title=Rewritten text:,
		colframe=blue,colback=red!5!white,
		breakable,
		leftrule=0mm, 
		bottomrule=0mm,
		rightrule=0mm,
		toprule=0mm,
		arc=0mm, outer arc=0mm,
		oversize
	}
}{
	\newenvironment{inserted}{}{}
	\let\deleted\comment
	\newenvironment{refactored}{}{} 
}

% ============================================================
% Put edit comments in a really ugly standout display
\newboolean{showcomments}
\setboolean{showcomments}{true}
%\setboolean{showcomments}{false}
\ifthenelse{\boolean{showcomments}}
{\newcommand{\nbc}[3]{
		{\colorbox{#3}{\bfseries\sffamily\scriptsize\textcolor{white}{#1}}}
		{\textcolor{#3}{\sf\small$\blacktriangleright$\textit{#2}$\blacktriangleleft$}}}
	\newcommand{\version}{\emph{\scriptsize\id}}}
{\newcommand{\nbc}[3]{}
	\newcommand{\version}{}}

% ============================================================
% Constants
\newcounter{qcounter}

% ============================================================================
% Make quotes be italic
\renewenvironment{quote}
{\list{}{\rightmargin\leftmargin}
	\item\relax\begin{it}}
	{\end{it}\endlist}
\newcommand{\ttimes}{\ensuremath{\times}}

% =============================================================================
% Source Code
\definecolor{source}{gray}{0.9}
\lstset{
	language={},
	% characters
	tabsize=3,
	upquote=true,
	escapechar={^},
	keepspaces=true,
	breaklines=false,
	alsoletter={},
	breakautoindent=true,
	columns=fullflexible,
	showstringspaces=false,
	basicstyle=\footnotesize\ttfamily,
	% background
	frame=single,
	framerule=0pt,
	backgroundcolor=\color{source},
	% numbering
	numbers=left,
	numbersep=5pt,
	numberstyle=\tiny,
	numberfirstline=true,
	% captioning
	captionpos=b,
	numberbychapter=false,
	% formatting (html)
	moredelim=[is][\textbf]{<b>}{</b>},
	moredelim=[is][\textit]{<i>}{</i>},
	moredelim=[is][\uline]{<u>}{</u>}}
\newcommand{\ct}{\lstinline[backgroundcolor=\color{white},basicstyle=\footnotesize\ttfamily]}
\newcommand{\lct}[1]{{\small\tt #1}}

%----------------------------------------------------------------------------
% Custom macros
\newcommand\keyword[1]{[#1]}

%----------------------------------------------------------------------------
% References
% \newcommand{\tabref}[1]{\hyperref[{tab:#1}]{Table~\ref*{tab:#1}}}
% \newcommand{\figref}[1]{\hyperref[{fig:#1}]{Figure~\ref*{fig:#1}}}
% \newcommand{\secref}[1]{\hyperref[{sec:#1}]{Section~\ref*{sec:#1}}}
% \newcommand{\lstref}[1]{\hyperref[{lst:#1}]{Listing~\ref*{lst:#1}}}
% \newcommand{\charef}[1]{\hyperref[{cha:#1}]{Chapter~\ref*{cha:#1}}}

%----------------------------------------------------------------------------
% Abbreviations
\tracingcolors 4
\setcounter{tocdepth}{3}
\setcounter{secnumdepth}{3}

\newcommand{\newevenside}{
	\ifthenelse{\isodd{\thepage}}{\newpage}{
		\newpage
		\phantom{placeholder} % doesn't appear on page
		\thispagestyle{empty} % if want no header/footer
		\newpage
	}
}

\def\stretchfactor{1}
\newcommand{\mychapter}[1]{\setstretch{1}
	\chapter{#1}\setstretch{\stretchfactor}}

\newcommand{\lessSpace}{\vspace{-1em}}
\DeclareGraphicsExtensions{.pdf,.png}
\graphicspath{{images/}}
\newcommand{\fig}[4]{
	\begin{figure}[#1]
		\centering
		\includegraphics[width=#2\textwidth]{#3}
		\lessSpace
		\caption{\label{fig:#3}#4}
\end{figure}}


\theoremstyle{definition}
\newtheorem{definition}{Definition}
\newcommand{\defref}[1]{\hyperref[{def:#1}]{Definition~\ref*{def:#1}}}

\newcommand{\columbo}{\textsc{Columbo}\xspace}

% ===========================================================================
% Front Page

% \newcommand{\thesistitle}{Web Communication Analysis\\of Android Applications}
% \newcommand{\thesisauthor}{Marc-Andrea Tarnutzer}
% \newcommand{\thesisauthorOrigin}{Basel BS, Switzerland}
% \newcommand{\thesisleiter}{Prof.\ Dr.\ Oscar Nierstrasz}
% \newcommand{\thesisasst}{Pascal Gadient}
% \newcommand{\thesisurl}{http://scg.unibe.ch/}
% \newcommand{\thesissubtitle}{}
% %Analysis of Common Issues
% \newcommand{\thesisdate}{26 April 2019}

% \newcommand{\hrref}[2]{\hyperref}

% \begin{document}
% \hypersetup{pageanchor=false}
% \begin{titlepage}  
% \begin{center}  

% \begin{figure}[t]  
% \vspace*{-2cm}        % to move header logo at the top 
% \center{\includegraphics[scale=1.2]{logos/MSc_quer.pdf}}
% \vspace{0.2in}     
% \end{figure}

% \thispagestyle{empty}

% {\bfseries\Huge \thesistitle \par
% \Large \thesissubtitle \par}

% \vspace{0.3in} 
% \LARGE{\textbf{Master Thesis} \\}
% \vspace{0.4in}

% {\Large \thesisauthor \par from \\\thesisauthorOrigin}

% \vspace{0.3in}
% {\Large Faculty of Science\\
% at the University of Bern\par}
% \vspace{0.3in}
% {\Large \thesisdate \par}
% \vspace{0.3in}

% {\Large \thesisleiter} \\
% {\Large \thesisasst} \par
% \vspace{0.3in}
% {\Large Software Composition Group\\}
% {\Large Institute for Computer Science\par University of Bern, Switzerland \par}

% \vspace{0.3in}

% \begin{figure}[htp]
% \centering
% \includegraphics[scale=0.40,trim=2cm 2cm 2cm 2cm]{logos/UNI_Bern.pdf}\hfill
% \includegraphics[scale=0.55]{logos/UNI_Neuenburg.eps}\hfill
% \includegraphics[scale=0.90]{logos/UNI_Fribourg.eps}
% \end{figure}

% \end{center}

% \end{titlepage}
% \hypersetup{pageanchor=true}


%\pagestyle{headings}
% \frontmatter

% Add space to making text easier to read
% \onehalfspacing

% ============================================================
\newboolean{isblinded}
\setboolean{isblinded}{false}
%\setboolean{isblinded}{false}
\ifthenelse{\boolean{isblinded}}
{\newcommand\blind[1]{BLINDED\xspace}}
{\newcommand\blind[1]{#1\xspace}}
% ============================================================



==> tables/basic_uelements.tex <==
\begin{table}                                                                       
\centering                                                                          
\caption{Overview of essential UAST interfaces}
\begin{tabularx}{\textwidth}{|X|X|}
\hline \textbf{UAST Interface} & \textbf{Purpose}\\    
\hline            
\code{UElement} & Basic interface for all UAST elements.\\    
\hline
\code{UResolvable} & Represents a \code{UElement} that references another element in the code, like a method call or a used variable which both reference their declaration.
Provides the \code{resolve} method to retrieve the referenced PSI element.\\
\hline
\code{UDeclaration} & Generic interface for all declarations: Classes, methods and variables.\\
\hline
\code{UClass} & Declaration of a class.
Provides access to all further declarations, like methods and variables, within the class.\\
\hline
\code{UMethod} & Declaration of a method.
Provides access to method parameters and body.\\
\hline
\code{UExpression} & Represents anything that can be evaluated like expressions and statements.\\
\hline
\code{UCallExpression} & Represents any method, constructor, or initializer call, and provides methods to gain access to the receiver, the arguments, and the called method.\\ \hline
\code{ULoopExpression} & Generic interfaces for all \code{for} and \code{while} loops.\\ \hline
\code{UForExpression} & Represents a \code{for} loop.\\ \hline
\code{UWhileExpression} & Represents a \code{while} loop.\\ \hline
\code{UForEachExpression} & Represents a \code{for} loop used to iterate over a collection of objects with the colon (\code{:}) notation.\\ \hline
\code{UReferenceExpression} & Represents any type of reference.\\ \hline
\code{USimpleNameReferenceExpression} & Represents plain, non-qualified identifiers.\\ \hline

\end{tabularx}                                                                       
\label{table:basic_uelements}                                                
\end{table}  
